What Must a Model Tell a Planner? Outcome Interfaces for Risk-Aware Planning After Robot Damage

When a robot is damaged, it must decide which routes it can still afford, and the amount of risk it may accept can change from one mission to the next. We argue that whether a learned model helps such a robot depends on its decision interface, that is, on what the model hands to the planner. A decision policy tells the planner what to do, whereas an outcome model, a kind of world model, predicts the consequences of each route. We study simulated Unitree Go2 quadrupeds and H1 humanoids with weakened motors, added payloads, or reduced foot friction. We compare four interfaces. The first is a decision policy, and the second is the same policy trained with fixed penalties for infeasible routes. The third is an outcome model that predicts the feasibility and travel time of each route. The fourth, which we call a capability contract, is an outcome model that predicts the chance of success and the travel time of the robot on each terrain and composes them along a route. All share the same collected experience, matched tuning and risk calibration, and an uncertainty guard. Two comparatively low-risk probes let the capability contract rank hazardous terrains about as well as four new trials on every hazard. At a calibrated 5% limit on selecting empirically infeasible routes, outcome models cut declined missions from about 32% to 7-8% on Go2 and from 57% to 35-36% on H1 compared with the plain policy. Fixed penalties narrow this gap, but the best penalty changes with the risk target. Predicting outcomes lets the planner preserve missions by changing routes as risk requirements tighten.

==> tab_h2h_full_rows.tex <==
Familiar, no target & Go2 & 6.5 (7.7) & 5.3 & 9.5 (10.9) & 4.4 & 1/20 & 9.5 & 4.3 \\
Familiar, no target & H1 & 13.5 (14.7) & 16.0 & 17.9 (20.0) & 12.7 & 0/20 & 17.7 & 12.7 \\
Familiar, $\alpha=10\%$ & Go2 & 5.9 (7.0) & 6.9 & 8.2 (9.5) & 8.7 & 14/20 & 8.2 & 8.7 \\
Familiar, $\alpha=10\%$ & H1 & 9.4 (11.5) & 22.3 & 10.3 (11.3) & 32.4 & 20/20 & 10.4 & 31.5 \\
Familiar, $\alpha=5\%$ & Go2 & 2.8 (3.9) & 7.7 & 3.5 (4.7) & 31.8 & 20/20 & 3.5 & 31.8 \\
Familiar, $\alpha=5\%$ & H1 & 4.1 (5.7) & 36.4 & 4.5 (5.8) & 56.6 & 20/20 & 4.6 & 55.5 \\
Familiar, $\alpha=2\%$ & Go2 & 0.6 (1.0) & 11.7 & 0.7 (1.3) & 60.7 & 20/20 & 0.7 & 61.0 \\
Familiar, $\alpha=2\%$ & H1 & 1.0 (1.6) & 59.9 & 1.2 (2.0) & 81.8 & 20/20 & 1.2 & 80.2 \\
New combinations, no target & Go2 & 6.6 (7.7) & 5.1 & 9.8 (12.8) & 4.3 & 1/20 & 9.8 & 4.3 \\
New combinations, no target & H1 & 13.2 (14.2) & 16.4 & 20.7 (22.1) & 12.5 & 0/20 & 20.9 & 12.8 \\
New combinations, $\alpha=5\%$ & Go2 & 2.7 (3.9) & 7.5 & 1.8 (3.2) & 49.2 & 20/20 & 1.8 & 49.1 \\
New combinations, $\alpha=5\%$ & H1 & 4.3 (5.5) & 35.4 & 2.0 (3.3) & 82.0 & 20/20 & 2.1 & 81.3 \\
Beyond the population, $\alpha=5\%$ & Go2 & 3.5 (5.7) & 46.6 & 3.5 (5.1) & 60.5 & 20/20 & 3.4 & 60.8 \\


==> tab_ident_rows.tex <==
Stale pre-damage model & 0 & 0.00 & 0.60 & $-44$ & 0 & 0.00 & 0.61 & $-61$ \\
Population average & 0 & 0.00 & 0.67 & 0 & 0 & 0.00 & 0.75 & 0 \\
Two flat probes & 2 & 0.01 & 0.81 & 20 & 2 & 0.00 & 0.84 & 25 \\
Two designed probes (ours) & 2 & 0.05 & 0.87 & 48 & 2 & 0.07 & 0.86 & 29 \\
Re-test each hazard $4\times$ & 36 & 17.5 & 0.87 & 44 & 32 & 15.9 & 0.85 & 20 \\
Re-test each hazard $8\times$ & 72 & 36.1 & 0.89 & 52 & 64 & 31.4 & 0.87 & 22 \\


==> tab_route_full_rows.tex <==
Familiar, no target & Go2 & 5.3 & 78.0 & 9.6 (11.2) & 4.3 & 78.3 & 1/20 \\
Familiar, no target & H1 & 16.0 & 65.6 & 16.8 (18.4) & 13.0 & 66.6 & 1/20 \\
Familiar, $\alpha=10\%$ & Go2 & 6.9 & 77.3 & 7.4 (8.7) & 6.5 & 78.1 & 2/20 \\
Familiar, $\alpha=10\%$ & H1 & 22.3 & 62.9 & 9.7 (11.6) & 21.4 & 63.2 & 6/20 \\
Familiar, $\alpha=5\%$ & Go2 & 7.7 & 74.1 & 2.8 (4.0) & 7.1 & 75.9 & 2/20 \\
Familiar, $\alpha=5\%$ & H1 & 36.4 & 54.1 & 4.5 (6.0) & 34.9 & 54.4 & 6/20 \\
Familiar, $\alpha=2\%$ & Go2 & 11.7 & 64.6 & 0.5 (1.1) & 10.6 & 65.8 & 4/20 \\
Familiar, $\alpha=2\%$ & H1 & 59.9 & 38.7 & 0.9 (2.0) & 71.5 & 30.9 & 12/20 \\
New combinations, no target & Go2 & 5.1 & 78.5 & 9.8 (10.9) & 4.3 & 78.1 & 1/20 \\
New combinations, no target & H1 & 16.4 & 65.8 & 17.8 (19.3) & 13.1 & 64.3 & 2/20 \\
New combinations, $\alpha=5\%$ & Go2 & 7.5 & 74.7 & 2.3 (3.4) & 7.1 & 75.1 & 4/20 \\
New combinations, $\alpha=5\%$ & H1 & 35.4 & 55.5 & 3.8 (5.5) & 39.3 & 48.4 & 18/20 \\
Beyond the population, $\alpha=5\%$ & Go2 & 46.6 & 75.0 & 4.4 (6.6) & 44.8 & 76.2 & 2/20 \\


==> tab_value_rows.tex <==
Stale pre-damage model & $-521$ & $-44$ & $-28$ & $-227$ & $-61$ & $-48$ \\
Two flat probes & $-18$ & 20 & 25 & 17 & 25 & 22 \\
Two designed probes (ours) & 25 & 48 & 49 & 19 & 29 & 27 \\
Re-test each hazard $4\times$ & 2 & 44 & 39 & 9 & 20 & 15 \\
Re-test each hazard $8\times$ & 21 & 52 & 45 & 10 & 22 & 18 \\

